Castelnuovo's bound and rigidity in almost complex geometry

This article is concerned with the question of whether an energy bound implies a genus bound for pseudo-holomorphic curves in almost complex manifolds. After reviewing what is known in dimensions other than 6, we establish a new result in this direction in dimension 6; in particular, for symplectic Calabi-Yau 6-manifolds. The proof relies on compactness and regularity theorems for J-holomorphic currents.

==> NormalCauchyRiemannOperator.tex <==
\section{The normal Cauchy--Riemann operator}
\label{Sec_NormalCauchyRiemannOperator}

The normal Cauchy--Riemann operator for embedded $J$--holomorphic maps can be traced back to the work of \citet[2.1.B]{Gromov1985}.
It was observed by \citet[Section 1.3]{Ivashkovich1999},
and \citet[Section 3]{Wendl2010}
that normal Cauchy--Riemann operator can be defined even for non-embedded $J$--holomorphic maps,
and that it plays an important role in understanding the deformation theory of $J$--holomorphic curves.
In this section we will briefly explain the construction of $Tu$ and $Nu$, and discuss the proof of \autoref{Prop_DDelbarVSDN}.

Let $u\co (\Sigma,j) \to (M,J)$ be a non-constant $J$--holomorphic map.
Denote by $\fd_{u,J}$ the real Cauchy--Riemann operator on $u^*TM$.
Denote by $\delbar_{u,J}$ the complex linear part of $\fd_{u,J}$.
This is a complex Cauchy--Riemann operator and gives $u^*TM$ the structure of a holomorphic vector bundle
\begin{equation*}
  \sE \coloneq (u^*TM,\delbar_{u,J}).
\end{equation*}
Denote by $\sT\Sigma$ the tangent bundle of $\Sigma$ equipped with its natural holomorphic structure.
The derivatives of $u$ induce a holomorphic map $\rd u \co \sT\Sigma \to \sE$.
The quotient of this map, thought of as a morphism of sheaves, 
\begin{equation*}
  \sQ \coloneq \sE/\sT\Sigma
\end{equation*}
is a coherent sheaf on $\Sigma$.
It is locally free outside the critical points of $\rd u$.
Denote by $D$ the divisor of the critical points of $\rd u$, counted with multiplicity.  
Near a critical point $z_0$ of order $k$ we can write $\rd u$ as $(z-z_0)^kf(z)$ with $f(z_0) \neq 0$.
Consequently, the torsion subsheaf of $\sQ$ is $\sO_D$,
the structure sheaf of $D$.
The quotient sheaf
\begin{equation*}
  \sN\!u \coloneq \sQ/\sO_D
\end{equation*}
is torsion free, and so locally free because $\dim_\C \Sigma = 1$; 
that is, $\sN\!u$ is a holomorphic vector bundle.
Similarly, the sheaf
\begin{equation*}
  \sT\!u \coloneq \ker(\sE \to \sN\!u)
\end{equation*}
is locally free.
We call $\sN\!u$ the \defined{generalized normal bundle} of $u$ and $\sT\!u$ the \defined{generalized tangent bundle} of $u$.

\begin{prop}
  We have
  \begin{equation*}
    \sT\!u/\sT\Sigma \iso \sO_D \qandq
    \sT\!u \iso \sT \Sigma(D).
  \end{equation*}
\end{prop}

\begin{proof}
  The following commutative diagram summarizes the construction of $\sT\!u$ and $\sN\!u$:
  \begin{equation*}
    \begin{tikzcd}
      &  & \sO_D \ar[d,hook] \\
      \sT\Sigma \ar[r,hook] \ar[d,hook] & \sE \ar[d,"="] \ar[r,two heads] & \sQ \ar[d,two heads] \\
      \sT\!u \ar[r,hook] \ar[d,two heads] & \sE \ar[r,two heads] & \sN\!u \\
      \sT\!u/\sT\Sigma.
    \end{tikzcd}
  \end{equation*}
  Since the columns and rows are exact sequences,
  it follows from the Snake Lemma that
  \begin{equation*}
    \sO_D \iso \sT\!u/\sT\Sigma.
  \end{equation*}
  This implies the assertion.
\end{proof}

\begin{proof}[Proof of \autoref{Prop_DDelbarVSDN}]
  Let $\sS$ be an $\Aut(\Sigma,j)$--invariant local slice around $j$ of the Teichmüller space $\sT(\Sigma)$.
  Recall that $\rd_{u,j}\delbar_J \co \Gamma(u^*TM)\oplus T_j\sS \to \Omega^{0,1}(\Sigma,u^*TM)$ is the linearization of $\delbar_J$,
  defined in \eqref{Eq_JHolomorphic},
  restricted to $C^\infty(\Sigma,M)\times \sS$.
  Denote by $Tu$ the complex vector bundle underlying $\sT\!u$ and by $Nu$ the complex vector bundle underlying $\sN\!u$.
  As was mentioned before \autoref{Def_NormalCauchyRiemannOperator},
  $Tu \subset u^*TM$ is the unique complex subbundle of rank one containing $\rd u(T\Sigma)$.
  Using a Hermitian metric on $u^*TM$ we obtain an isomorphism
  \begin{equation*}
    u^*TM \iso Tu \oplus Nu.
  \end{equation*}
  With respect to this splitting $\fd_{J,u}$,
  the restriction of $\rd_{u,j}\delbar_J$ to $\Gamma(u^*TM)$,
  can be written as
  \begin{equation*}
    \fd_{J,u}
    =
    \begin{pmatrix}
      \fd_{u,J}^T & * \\
      \dagger & \fd_{u,J}^N
    \end{pmatrix}
  \end{equation*}
  with $\fd_{u,J}^N$ denoting the normal Cauchy--Riemann operator introduced in \autoref{Def_NormalCauchyRiemannOperator}.
  Since
  \begin{equation*}
    \delbar_{u,J}\circ \rd u = \rd u \circ \delbar_{T\Sigma}
    \qandq
    \sT\!u \iso \sT\Sigma(D),
  \end{equation*}
  it follows that
  \begin{equation*}
    \delbar_{u,J}^T = \delbar_{Tu} \qandq \dagger = 0.
  \end{equation*}
  Denote by $\iota \co T_j\sS \to \Omega^{0,1}(\Sigma,u^*TM)$ the restriction of $\rd_{u,j}\delbar_J$ to $T_j\sS$.
  The tangent space to the Teichmüller space $\sT(\Sigma)$ at $[j]$ can be identified with $\coker \delbar_{T\Sigma} \iso \ker \delbar_{T\Sigma}^*$.
  With respect to this identification,
  $\iota$ is the restriction of $\rd u\co T\Sigma \to u^*TM$ to $\ker \delbar_{T\Sigma}^*$.
  Consequently,
  we can write $\rd_{u,j}\delbar_J \co \Gamma(Tu)\oplus T_j\sS \oplus \Gamma(Nu) \to \Gamma(Tu)\oplus\Gamma(Nu)$ as
  \begin{equation*}
    \rd_{u,j}\delbar_J
    =
    \begin{pmatrix}
      \delbar_{Tu} & \iota & *\\
      0 & 0 & \fd_{u,J}^N
    \end{pmatrix}.
  \end{equation*}

  The short exact sequence
  \begin{equation*}
    0 \to \sT\Sigma \to \sT\!u \to \sO_D \to 0
  \end{equation*}
  induces the following long exact sequence in cohomology
  \begin{equation*}
    0 \to H^0(\sT\Sigma) \to H^0(\sT\!u) \to H^0(\sO_D) \to H^1(\sT\Sigma) \to H^1(\sT\!u) \to 0.
  \end{equation*}
  It follows that
  \begin{equation*}
    \ind \delbar_{Tu}
    = 2\chi(\sT\!u)
    = 2\chi(\sT\Sigma) + 2h^0(\sO_D)
    = \ind \delbar_{T\Sigma} + 2Z(\rd u),
  \end{equation*}
  that $\ker \delbar_{T\Sigma} \to \ker \delbar_{Tu}$ is injective,
  and that $\coker \delbar_{T\Sigma} \to \coker \delbar_{Tu}$ is surjective.
  The latter implies that $\delbar_{Tu} \oplus \iota$ is surjective.
  Therefore,
  there are an exact sequence
  \begin{equation*}
    0 \to \ker \delbar_{Tu} \oplus \iota \to \ker \rd_{u,j}\delbar_J  \to \ker \fd_{u,J}^N \to 0,
  \end{equation*}
  and an isomorphism
  \begin{equation*}
    \coker \rd_{u,j}\delbar_J \iso \coker \fd_{u,J}^N.
  \end{equation*}
  The kernel of $\delbar_{Tu} \oplus \iota$ contains $\aut(\Sigma,j) = \ker \delbar_{T\Sigma}$ and
  \begin{align*}
    \dim\ker \delbar_{Tu}\oplus\iota
    &= \ind \delbar_{Tu}\oplus\iota \\
    &= \ind \delbar_{Tu} + \dim T_j\sS \\
    &= \ind \delbar_{T\Sigma} + \dim T_j\sS + 2Z(\rd u) \\
    &= \dim \aut(\Sigma,j) + 2Z(\rd u).
  \end{align*}
  This completes the proof of \autoref{Prop_DDelbarVSDN}.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "SuperRigidityCastelnuovo"
%%% End:


==> Proofs.tex <==
\section{Proofs of \autoref{Prop_NoUniversalGenusBound} and \autoref{Prop_HighDimensionalCastelnuovo}}
\label{Sec_ProofsFromIntroduction}

% The following is a consequence of Gromov's h-principle for symplectic immersions \cite[Section 3.4.2 Theorem (A)]{Gromov1986} and Thom's theorem on representability of homology classes \cite[Théorème II.27]{Thom1954}; see also \cite[Corollary 2.13]{Li2005}.
% In higher dimensions there cannot be a genus bound which holds for all almost complex structures.

\begin{proof}[Proof of \autoref{Prop_NoUniversalGenusBound}]
  By a classic theorem of Thom \cite[Théorème II.27]{Thom1954},
  there is a closed, connected, oriented surface $\Sigma$ and an embedding $u_0\co \Sigma \to M$ with $u_*[\Sigma] = A$.
  After adding sufficiently many small $1$--handles,
  we can assume that $g(\Sigma) \geq n$.  
  Gromov's $h$--principle \cite[Section 3.4.2 Theorem (A)]{Gromov1986} implies that $u_0$ is $C^0$--close to an embedding $u\co \Sigma \to M$ with $u^*\omega > 0$.

  Denote the image of $u$ by $C$.
  The restriction of $TM$ to $C$ is the direct sum of the symplectic subbundle $TC$ and its symplectic complement, which can be identified with $NC$.
  The space of complex structures on $\R^{2n}$ compatible with a fixed non-degenerate $2$--form form is contractible.
  This implies that:
  \begin{enumerate*}[(1)]
  \item
    both $TC$ and $NC$ admit almost complex structures compatible with $\omega$;
    hence, $TM|_C$ admits an almost complex structure compatible with $\omega$,
    and 
  \item
    any such almost complex structure on $TM|_C$ can be extended to an almost complex structure on $TM$ compatible with $\omega$.
  \end{enumerate*}
\end{proof}

\begin{remark}  
  If $(M,\omega)$ is a symplectic $4$--manifold,
  then every $A \in H_2(M)$ with $\inner{[\omega]}{A} > 0$ is represented by an \emph{immersed} symplectic surface $C$ with transverse double points.
  Such a surface is $J$--holomorphic for an almost complex structure compatible with $\omega$ if only if all of its self-intersections are positive.
\end{remark}

\begin{proof}[Proof of \autoref{Prop_HighDimensionalCastelnuovo}]
  Denote by $\sM$ the component of the universal moduli space of simple pseudo-holomorphic maps from a Riemann surface of genus $g$ to $M$.
  This is a separable  Banach manifold and the projection map $\pi \co \sM \to \sJ$ is a Fredholm map of class $C^1$ and index
  \begin{equation*}
    (n-3)(2-2g) + 2\inner{c_1(M,J)}{A};
  \end{equation*}
  see, e.g., \cites[Proposition 3.2.1]{McDuff2012}[Section 7.5]{Wendl2016a}.
  If \autoref{Eq_HighDimensionalCastelnuovo} is violated,
  then this index is negative.
  The result thus follows from the Sard--Smale theorem \cite{Smale1965}.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "CastelnuovoRigidity"
%%% End:

